Advances in ArborX to support exascale applications

ArborX is a performance portable geometric search library developed as part of the Exascale Computing Project (ECP). In this paper, we explore a collaboration between ArborX and a cosmological simulation code HACC. Large cosmological simulations on exascale platforms encounter a bottleneck due to the in-situ analysis requirements of halo finding, a problem of identifying dense clusters of dark matter (halos). This problem is solved by using a density-based DBSCAN clustering algorithm. With each MPI rank handling hundreds of millions of particles, it is imperative for the DBSCAN implementation to be efficient. In addition, the requirement to support exascale supercomputers from different vendors necessitates performance portability of the algorithm. We describe how this challenge problem guided ArborX development, and enhanced the performance and the scope of the library. We explore the improvements in the basic algorithms for the underlying search index to improve the performance, and describe several implementations of DBSCAN in ArborX. Further, we report the history of the changes in ArborX and their effect on the time to solve a representative benchmark problem, as well as demonstrate the real world impact on production end-to-end cosmology simulations.

==> arborx.tex <==
\section{ArborX overview}\label{s:arborx}

In this Section, we give a brief introduction to geometric search algorithms
and the ArborX library, setting up a background for performance improvements in
\Cref{s:updates}.

The main index in ArborX is a bounding volume hierarchy (BVH). BVH is a tree
structure created from a set of objects in a multi-dimension space. Each object
is wrapped in a geometric format (\emph{bounding volume}) to form the leaf
nodes of the tree. Each node of a BVH is an aggregate of its children, with the
node's bounding volume enclosing the bounding volumes of its children. The
bounding volume around all objects, called \emph{scene bounding volume},
is stored at the root of the hierarchy.

As was demonstrated in \cite{karras2012}, binary BVH is a good
choice for GPU-based searches, particularly for low-dimensional data
typical in the scientific applications. Fast BVH construction algorithms use a
space-filling curve (Z-curve) to improve the spatial locality of the user data,
followed by a single bottom-up construction to produce a binary tree structure
(hierarchy). While the resulting quality is somewhat worse than produced by the
best available algorithms, the construction procedure is extremely fast and
produces a tree of sufficient quality in most situations.

During the search (also called a traversal), each thread \revision{(a host or a
GPU thread depending on the backend)} is assigned a single query,
\revision{\emph{i.e.}, a spatial or $k$-nearest neighbor search problem}. All
the traversals are performed independently in parallel in a top-down manner. To
reduce the data and thread divergence, the queries are pre-sorted with the goal
to assign neighboring threads the queries that are geometrically close.

To reduce the software development cost, ArborX uses Kokkos \citep{kokkos2022}
for on-node parallelism to allow running on a variety of commodity and HPC
hardware, including Nvidia, AMD, and Intel GPUs. Kokkos abstracts common
parallel execution patterns, such as parallel loops, reductions, and scans
(prefix sums), from the underlying hardware architecture.
In addition, Kokkos provides an abstraction for a multi-dimensional array data
structure called \texttt{View}. It is a polymorphic structure, whose layout
depends on the memory the data resides in (host or device).

Kokkos supports both CPUs and GPUs (Nvidia, AMD, Intel) through providing
backends, e.g., OpenMP, CUDA, SYCL, HIP. Using Kokkos allows running the same
code on CPUs or GPUs by simply changing the backend through a template
parameter, resulting in a higher developer productivity.

Now, we briefly describe the scope of different focus areas within ArborX.

\subsubsection*{Core functionality.}
ArborX supports two kinds of search types: range and nearest. The \emph{range}
search finds all objects that intersect with a query object. For example,
finding all objects within a certain distance is a range search. The
\emph{nearest} search, on the other hand, looks for a certain number of the
closest objects, regardless of their distance. Both searches support
multi-dimensional data, with dimensions ranging 1--10.

These two search types require very different tree traversal algorithms. The
range query has to explore all nodes in a tree that satisfy the given
predicate. It can be implemented in a stackless manner (see
\Cref{s:stackless}). In contrast, the nearest search can terminate early while
it has found the best possible candidates. Nearest search is more complicated
to implement, and relies on a stack and a priority queue structures.

ArborX provides both on-node and distributed (through using MPI)
implementations for both searches.

\subsubsection*{Clustering functionality.}
ArborX provides implementations for several clustering algorithms that depend
on distance calculations: \dbscan (the focus of this work) and Euclidean minimum
spanning tree \citep{prokopenko2023emst}. There are ongoing efforts to provide
an efficient implementation for the \hdbscan algorithm \citep{campello2015}.

\subsubsection*{Ray tracing functionality.}
ArborX provides basic support for ray tracing.

\subsubsection*{Interpolation functionality.}
ArborX implements moving least squares interpolation algorithm
\citep{quaranta2005}. In this method, support and subsequently the interpolation
operator are constructed through solving local least squares problems defined
by compactly supported radial basis functions.

